Effects on the local dark matter distribution due to the Large Magellanic Cloud

We study the local dark matter distribution in two models for the Milky Way (MW)-Large Magellanic Cloud (LMC) interaction. The effect of the LMC on the local dark matter distribution is dependent on the evolution of the MW-LMC system, such that a static model is insufficient to accurately model the dark matter velocity distribution in the solar neighbourhood. An evolved model boosts local LMC dark matter particle velocities by nearly 50%, to a median value of $\approx750$km/s. MW dark matter particles also experience a velocity boost, which we identify as being caused by reflex motion owing to the infall of the LMC. We study the implications of LMC particles in the solar neighbourhood for dark matter detection experiments. Specifically, the directionality of LMC particles is distinguishable from the MW particles, with a difference in the apparent origin centroid location between the MW and LMC particles of $26\pm6 ^\circ$. This unique identifier, along with their high velocities, can be utilised by directional detectors to search for dark matter particles originating in the LMC.

==> thebibliography.tex <==
\begin{thebibliography}{}
\makeatletter
\relax
\def\mn@urlcharsother{\let\do\@makeother \do\$\do\&\do\#\do\^\do\_\do\%\do\~}
\def\mn@doi{\begingroup\mn@urlcharsother \@ifnextchar [ {\mn@doi@}
  {\mn@doi@[]}}
\def\mn@doi@[#1]#2{\def\@tempa{#1}\ifx\@tempa\@empty \href
  {http://dx.doi.org/#2} {doi:#2}\else \href {http://dx.doi.org/#2} {#1}\fi
  \endgroup}
\def\mn@eprint#1#2{\mn@eprint@#1:#2::\@nil}
\def\mn@eprint@arXiv#1{\href {http://arxiv.org/abs/#1} {{\tt arXiv:#1}}}
\def\mn@eprint@dblp#1{\href {http://dblp.uni-trier.de/rec/bibtex/#1.xml}
  {dblp:#1}}
\def\mn@eprint@#1:#2:#3:#4\@nil{\def\@tempa {#1}\def\@tempb {#2}\def\@tempc
  {#3}\ifx \@tempc \@empty \let \@tempc \@tempb \let \@tempb \@tempa \fi \ifx
  \@tempb \@empty \def\@tempb {arXiv}\fi \@ifundefined
  {mn@eprint@\@tempb}{\@tempb:\@tempc}{\expandafter \expandafter \csname
  mn@eprint@\@tempb\endcsname \expandafter{\@tempc}}}

\bibitem[\protect\citeauthoryear{Akimov et~al.,}{Akimov
  et~al.}{2020}]{Akimov_2020}
Akimov D.,  et~al., 2020, \mn@doi [Physical Review D]
  {10.1103/physrevd.102.052007}, 102

\bibitem[\protect\citeauthoryear{Aprile et~al.,}{Aprile
  et~al.}{2017}]{Aprile_2017}
Aprile E.,  et~al., 2017, EPJ C, 77

\bibitem[\protect\citeauthoryear{{Bennett} \& {Bovy}}{{Bennett} \&
  {Bovy}}{2019}]{Bennett..2019}
{Bennett} M.,  {Bovy} J.,  2019, \mn@doi [\mnras] {10.1093/mnras/sty2813},
  \href {https://ui.adsabs.harvard.edu/abs/2019MNRAS.482.1417B} {482, 1417}

\bibitem[\protect\citeauthoryear{Besla, Peter  \& Garavito-Camargo}{Besla
  et~al.}{2019}]{Besla_2019}
Besla G.,  Peter A.,   Garavito-Camargo N.,  2019, \mn@doi [JCAP]
  {10.1088/1475-7516/2019/11/013}, 2019, 013–013

\bibitem[\protect\citeauthoryear{B{\oe}hm, Cerdeño, Machado, Campo  \&
  Reid}{B{\oe}hm et~al.}{2019}]{Boehm_2019}
B{\oe}hm C.,  Cerdeño D.,  Machado P.,  Campo A. O.-D.,   Reid E.,  2019,
  \mn@doi [JCAP] {10.1088/1475-7516/2019/01/043}, 2019, 043–043

\bibitem[\protect\citeauthoryear{Drukier, Freese  \& Spergel}{Drukier
  et~al.}{1986}]{Drukier_1986}
Drukier A.~K.,  Freese K.,   Spergel D.~N.,  1986, \mn@doi [Phys. Rev. D]
  {10.1103/PhysRevD.33.3495}, 33, 3495

\bibitem[\protect\citeauthoryear{{Eadie} \& {Juri{\'c}}}{{Eadie} \&
  {Juri{\'c}}}{2019}]{Eadie_2019}
{Eadie} G.,  {Juri{\'c}} M.,  2019, \mn@doi [\apj] {10.3847/1538-4357/ab0f97},
  \href {https://ui.adsabs.harvard.edu/abs/2019ApJ...875..159E} {875, 159}

\bibitem[\protect\citeauthoryear{{Eilers}, {Hogg}, {Rix}  \& {Ness}}{{Eilers}
  et~al.}{2019}]{Eilers..2019}
{Eilers} A.-C.,  {Hogg} D.~W.,  {Rix} H.-W.,   {Ness} M.~K.,  2019, \mn@doi
  [\apj] {10.3847/1538-4357/aaf648}, \href
  {https://ui.adsabs.harvard.edu/abs/2019ApJ...871..120E} {871, 120}

\bibitem[\protect\citeauthoryear{{Erkal} et~al.,}{{Erkal}
  et~al.}{2019}]{Erkal_2019}
{Erkal} D.,  et~al., 2019, \mn@doi [\mnras] {10.1093/mnras/stz1371}, \href
  {https://ui.adsabs.harvard.edu/abs/2019MNRAS.487.2685E} {487, 2685}

\bibitem[\protect\citeauthoryear{Evans, O'Hare  \& McCabe}{Evans
  et~al.}{2018}]{Evans_2018}
Evans N.~W.,  O'Hare C. A.~J.,   McCabe C.,  2018, PRD

\bibitem[\protect\citeauthoryear{Gonzalez-Garcia, Maltoni, Perez-Gonzalez  \&
  Funchal}{Gonzalez-Garcia et~al.}{2018}]{Gonzalez_Garcia_2018}
Gonzalez-Garcia M.~C.,  Maltoni M.,  Perez-Gonzalez Y.~F.,   Funchal R.~Z.,
  2018, \mn@doi [Journal of High Energy Physics] {10.1007/jhep07(2018)019},
  2018

\bibitem[\protect\citeauthoryear{{Gravity Collaboration} et~al.,}{{Gravity
  Collaboration} et~al.}{2021}]{Gravity..2021}
{Gravity Collaboration} et~al., 2021, \mn@doi [\aap]
  {10.1051/0004-6361/202040208}, \href
  {https://ui.adsabs.harvard.edu/abs/2021A&A...647A..59G} {647, A59}

\bibitem[\protect\citeauthoryear{Grothaus, Fairbairn  \& Monroe}{Grothaus
  et~al.}{2014}]{Grothaus_2014}
Grothaus P.,  Fairbairn M.,   Monroe J.,  2014, \mn@doi [Physical Review D]
  {10.1103/physrevd.90.055018}, 90

\bibitem[\protect\citeauthoryear{Harris et~al.,}{Harris et~al.}{2020}]{numpy}
Harris C.~R.,  et~al., 2020, \mn@doi [Nature] {10.1038/s41586-020-2649-2}, 585,
  357

\bibitem[\protect\citeauthoryear{Herzog-Arbeitman, Lisanti  \&
  Necib}{Herzog-Arbeitman et~al.}{2018}]{Herzog_Arbeitman_2018}
Herzog-Arbeitman J.,  Lisanti M.,   Necib L.,  2018, \mn@doi [JCAP]
  {10.1088/1475-7516/2018/04/052}, 2018, 052–052

\bibitem[\protect\citeauthoryear{Hunter}{Hunter}{2007}]{matplotlib}
Hunter J.~D.,  2007, \mn@doi [Computing in Science \& Engineering]
  {10.1109/MCSE.2007.55}, 9, 90

\bibitem[\protect\citeauthoryear{Kallivayalil, van~der Marel, Besla, Anderson
  \& Alcock}{Kallivayalil et~al.}{2013}]{Kallivayalil_2013}
Kallivayalil N.,  van~der Marel R.~P.,  Besla G.,  Anderson J.,   Alcock C.,
  2013, \mn@doi [ApJ] {10.1088/0004-637x/764/2/161}, 764, 161

\bibitem[\protect\citeauthoryear{Kluyver et~al.,}{Kluyver
  et~al.}{2016}]{jupyter}
Kluyver T.,  et~al., 2016, in Loizides F.,  Scmidt B.,  eds, Positioning and
  Power in Academic Publishing: Players, Agents and Agendas. IOS Press,
  Netherlands, pp 87--90, \url{https://eprints.soton.ac.uk/403913/}

\bibitem[\protect\citeauthoryear{Lewin \& Smith}{Lewin \&
  Smith}{1996}]{Lewin_1996}
Lewin J.,  Smith P.,  1996, \mn@doi [Astroparticle Physics]
  {https://doi.org/10.1016/S0927-6505(96)00047-3}, 6, 87

\bibitem[\protect\citeauthoryear{Necib, Lisanti  \& Belokurov}{Necib
  et~al.}{2019}]{Necib_2019}
Necib L.,  Lisanti M.,   Belokurov V.,  2019, \mn@doi [ApJ]
  {10.3847/1538-4357/ab095b}, 874, 3

\bibitem[\protect\citeauthoryear{Nygren}{Nygren}{2013}]{Nygren_2013}
Nygren D.,  2013, \mn@doi [Journal of Physics Conference Series]
  {10.1088/1742-6596/460/1/012006}, 460, 2006

\bibitem[\protect\citeauthoryear{O’Hare, Evans, McCabe, Myeong  \&
  Belokurov}{O’Hare et~al.}{2020}]{O_Hare_2020_substructure}
O’Hare C.~A.,  Evans N.~W.,  McCabe C.,  Myeong G.,   Belokurov V.,  2020,
  \mn@doi [Physical Review D] {10.1103/physrevd.101.023006}, 101
  
\bibitem[\protect\citeauthoryear{O’Hare}{O’Hare}{2020}]{O_Hare_2020}
O’Hare C.~A.,  2020, \mn@doi [Physical Review D]
  {10.1103/physrevd.102.063024}, 102

\bibitem[\protect\citeauthoryear{P\'erez \& Granger}{P\'erez \&
  Granger}{2007}]{ipython}
P\'erez F.,  Granger B.~E.,  2007, \mn@doi [Computing in Science and
  Engineering] {10.1109/MCSE.2007.53}, 9, 21

\bibitem[\protect\citeauthoryear{{Petersen}, {Katz}  \& {Weinberg}}{{Petersen}
  et~al.}{2016}]{Petersen_2016}
{Petersen} M.~S.,  {Katz} N.,   {Weinberg} M.~D.,  2016, \mn@doi [\prd]
  {10.1103/PhysRevD.94.123013}, \href
  {https://ui.adsabs.harvard.edu/abs/2016PhRvD..94l3013P} {94, 123013}
  
  \bibitem[\protect\citeauthoryear{{Petersen} \& {Pe{\~n}arrubia}}{{Petersen} \&
  {Pe{\~n}arrubia}}{2020}]{Petersen..reflexmotion..2020}
{Petersen} M.~S.,  {Pe{\~n}arrubia} J.,  2020, \mn@doi [\mnras]
  {10.1093/mnrasl/slaa029}, \href
  {https://ui.adsabs.harvard.edu/abs/2020MNRAS.494L..11P} {494, L11}

\bibitem[\protect\citeauthoryear{Petersen \& Peñarrubia}{Petersen \&
  Peñarrubia}{2021}]{Petersen_2021_reflex_motion}
Petersen M.,  Peñarrubia J.,  2021, \mn@doi [Nature Astronomy]
  {10.1038/s41550-020-01254-3}, 5, 1

\bibitem[\protect\citeauthoryear{{Petersen}, {Weinberg}  \& {Katz}}{{Petersen}
  et~al.}{2021}]{Petersen_2021_commensurabilities}
{Petersen} M.~S.,  {Weinberg} M.~D.,   {Katz} N.,  2021, \mn@doi [\mnras]
  {10.1093/mnras/staa3202}, \href
  {https://ui.adsabs.harvard.edu/abs/2021MNRAS.500..838P} {500, 838}

\bibitem[\protect\citeauthoryear{{Petersen}, {Weinberg}  \& {Katz}}{{Petersen}
  et~al.}{2022}]{Petersen..EXP..2021}
{Petersen} M.~S.,  {Weinberg} M.~D.,   {Katz} N.,  2022, \mn@doi [\mnras]
  {10.1093/mnras/stab3639}, \href
  {https://ui.adsabs.harvard.edu/abs/2022MNRAS.510.6201P} {510, 6201}

\bibitem[\protect\citeauthoryear{Peñarrubia, Gómez, Besla, Erkal  \&
  Ma}{Peñarrubia et~al.}{2015}]{Penarrubia_2015}
Peñarrubia J.,  Gómez F.~A.,  Besla G.,  Erkal D.,   Ma Y.-Z.,  2015, \mn@doi
  [MNRASL] {10.1093/mnrasl/slv160}, 456, L54–L58

\bibitem[\protect\citeauthoryear{Pietrzyński et~al.,}{Pietrzyński
  et~al.}{2019}]{Pietrzynski_2019}
Pietrzyński G.,  et~al., 2019, \mn@doi [Nature] {10.1038/s41586-019-0999-4},
  567, 200–203

\bibitem[\protect\citeauthoryear{{Sch{\"o}nrich}, {Binney}  \&
  {Dehnen}}{{Sch{\"o}nrich} et~al.}{2010}]{Schonrich..2010}
{Sch{\"o}nrich} R.,  {Binney} J.,   {Dehnen} W.,  2010, \mn@doi [\mnras]
  {10.1111/j.1365-2966.2010.16253.x}, \href
  {https://ui.adsabs.harvard.edu/abs/2010MNRAS.403.1829S} {403, 1829}

\bibitem[\protect\citeauthoryear{{Weinberg}}{{Weinberg}}{1999}]{Weinberg..1999}
{Weinberg} M.~D.,  1999, \mn@doi [\aj] {10.1086/300669}, \href
  {https://ui.adsabs.harvard.edu/abs/1999AJ....117..629W} {117, 629}

\bibitem[\protect\citeauthoryear{{Zwicky}}{{Zwicky}}{1937}]{Zwicky_1937}
{Zwicky} F.,  1937, \mn@doi [\apj] {10.1086/143864}, \href
  {https://ui.adsabs.harvard.edu/abs/1937ApJ....86..217Z} {86, 217}


\bibitem[\protect\citeauthoryear{{van der Marel}, {Alves}, {Hardy}  \&
  {Suntzeff}}{{van der Marel} et~al.}{2002}]{vanderMarel_2002}
{van der Marel} R.~P.,  {Alves} D.~R.,  {Hardy} E.,   {Suntzeff} N.~B.,  2002,
  \mn@doi [\aj] {10.1086/343775}, \href
  {https://ui.adsabs.harvard.edu/abs/2002AJ....124.2639V} {124, 2639}

\bibitem[\protect\citeauthoryear{{van der Marel} \& {Kallivayalil}}{{van der
  Marel} \& {Kallivayalil}}{2014}]{vanderMarel_2014}
{van der Marel} R.~P.,  {Kallivayalil} N.,  2014, \mn@doi [\apj]
  {10.1088/0004-637X/781/2/121}, \href
  {https://ui.adsabs.harvard.edu/abs/2014ApJ...781..121V} {781, 121}


\makeatother
\end{thebibliography}
